PerfCodeBench: Benchmarking LLMs for System-Level High-Performance Code Optimization

Large language models (LLMs) can often generate functionally correct code, but their ability to produce efficient implementations for performance-critical systems tasks remains limited. Existing code benchmarks mainly emphasize correctness or algorithmic problem solving, while realistic systems-level optimization is still underexplored. To address this gap, we introduce PerfCodeBench, an executable benchmark for evaluating LLMs on high-performance code optimization. The tasks require system-level implementation choices, hardware-aware optimization, and careful handling of performance bottlenecks. Each task includes executable correctness checks, a baseline implementation, and a reference optimized solution. This allows us to evaluate both correctness and runtime-oriented efficiency. Our evaluation on a broad set of state-of-the-art LLMs shows a clear gap between model-generated code and expert-optimized implementations. The gap is especially large on tasks involving parallelism and GPU operations. Current models also show weaknesses in cross-language robustness and in consistently reaching expert-level efficiency. These results suggest that performance-aware evaluation are still needed. LLMs should move beyond generating merely correct code toward producing efficient systems software. We submit the benchmark data, evaluation infrastructure, and complete logs of all LLMs-generated code at https://anonymous.4open.science/r/perfcodebench-7CDE.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The abstract and introduction describe PerfCodeBench as an executable benchmark for system-level code optimization, and the claims are supported by the benchmark construction, evaluation metrics, and experimental results reported in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper discusses limitations related to executable benchmark coverage, dependence on available public systems sources, hardware-specific evaluation, and the cost of large-scale runtime measurement.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions.
        \item The authors should reflect on the scope of the claims made.
        \item The authors should reflect on the factors that influence the performance of the approach.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper introduces an executable benchmark and empirical evaluation pipeline. It does not present theoretical results or formal proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material.
    \end{itemize}

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper describes the task format, evaluation metrics, executable harness design, caching strategy, timeout calibration, and model evaluation protocol. We also submit the benchmark data, evaluation infrastructure, and complete evaluation logs for model-generated code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
    \end{itemize}

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}.
    \item[] Justification: We submit the benchmark data, evaluation infrastructure, and complete evaluation logs for all model-generated code in an anonymized repository. The repository includes the task data and scripts needed to run the executable evaluation pipeline.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible.
        \item The instructions should contain the exact command and environment needed to run to reproduce the results.
    \end{itemize}

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details necessary to understand the results?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper specifies the benchmark size, programming languages, task structure, correctness checks, runtime-based evaluation metrics, repeated execution protocol, adaptive timeout setting, and model list. Since the paper evaluates existing LLMs rather than training new models, optimizer and training hyperparameters are not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}.
    \item[] Justification: We do not report statistical significance tests across model runs because each model evaluation is expensive and involves executable compilation, correctness checking, and repeated runtime measurement across thousands of tasks. To reduce runtime noise, task performance is measured with repeated executions and median runtime aggregation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests.
        \item The factors of variability that the error bars are capturing should be clearly stated.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources needed to reproduce the experiments?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper describes the local executable benchmarking environment and distinguishes CPU and CUDA task pools. It also explains caching, adaptive timeouts, and workload-aware scheduling, which are needed to estimate and reproduce the evaluation cost.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The work evaluates code optimization ability using public code sources and executable benchmarks. We do not collect private user data, conduct human-subject studies, or release models with high misuse risk.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity.
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper discusses that better code optimization benchmarks can improve software efficiency and reduce resource consumption. It also notes that stronger code-generation models may produce flawed or unsafe optimized code if used without testing, making executable validation important.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses, fairness considerations, privacy considerations, and security considerations.
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper releases benchmark tasks, evaluation code, and model-generated code logs rather than a new generative model or high-risk scraped dataset. The benchmark focuses on executable performance optimization tasks from public systems sources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards.
        \item Datasets that have been scraped from the Internet could pose safety risks.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets used in the paper properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper cites the public repositories, benchmark suites, and project pages used as data sources. The appendix lists representative sources and reference links; the released artifact includes license and provenance information where applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license should be included for each asset.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}.
    \item[] Justification: PerfCodeBench is a new benchmark asset. We provide documentation for the task format, evaluation pipeline, metrics, and model-generated code logs in the submitted artifact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates.
        \item At submission time, remember to anonymize your assets if applicable.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine.
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether IRB approvals were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve human subjects, crowdsourcing participants, or user studies.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval may be required for any human subjects research.
        \item For initial submissions, do not include any information that would break anonymity.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerYes{}.
    \item[] Justification: LLMs are the objects of evaluation in this paper. The paper lists the evaluated models and describes the OpenAI-compatible inference interface used to obtain model-generated code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> texs/large_table.tex <==




\begin{table*}[t]
\centering
\tiny
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc cccccc cccccc cccccc cccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} 
& \multicolumn{6}{c}{\textbf{CRR(\%)}} 
& \multicolumn{6}{c}{\textbf{FBR(\%)}} 
& \multicolumn{6}{c}{\textbf{RBR(\%)}} 
& \multicolumn{6}{c}{\textbf{CGRE(\%)}} 
& \multicolumn{6}{c}{\textbf{CGRE$_{\ge 0.8}$(\%)}} \\
\cmidrule(lr){2-7}
\cmidrule(lr){8-13}
\cmidrule(lr){14-19}
\cmidrule(lr){20-25}
\cmidrule(lr){26-31}
& C & C++ & Go & Java & Py & CUDA
& C & C++ & Go & Java & Py & CUDA
& C & C++ & Go & Java & Py & CUDA
& C & C++ & Go & Java & Py & CUDA
& C & C++ & Go & Java & Py & CUDA \\
\midrule

GPT-5.4 
& 58.02 & 86.84 & 85.00 & 81.82 & 98.61 & 2.40
& 53.70 & 82.24 & 75.00 & 77.84 & 65.28 & 0.00
& 33.33 & 65.59 & 41.09 & 56.40 & 50.85 & 0.00
& 38.26 & 80.78 & 78.36 & 75.00 & 70.93 & 0.00
& 34.06 & 78.27 & 79.07 & 73.26 & 66.95 & 0.00 \\

\midrule

GPT-5 
& 32.72 & 73.78 & 81.88 & 84.09 & 82.64 & 9.60
& 29.63 & 71.67 & 78.75 & 81.82 & 70.14 & 5.60
& 21.01 & 62.44 & 55.81 & 57.56 & 66.10 & 0.00
& 24.65 & 71.47 & 77.45 & 79.32 & 70.82 & 6.70
& 22.46 & 70.64 & 78.29 & 76.74 & 67.80 & 6.86 \\

Claude Opus 4.5 
& 58.02 & 83.07 & 86.88 & 89.20 & 81.25 & 12.00
& 51.23 & 77.92 & 78.75 & 86.93 & 70.14 & 8.80
& 31.88 & 51.76 & 35.66 & 61.05 & 57.63 & 0.00
& 37.54 & 76.87 & 78.65 & 81.77 & 72.52 & 10.26
& 34.06 & 74.93 & 79.84 & 76.16 & 71.19 & 10.78 \\

\midrule

Claude Sonnet 4.5 
& 56.17 & 86.02 & 72.50 & 75.00 & 87.50 & 9.60
& 45.68 & 77.28 & 67.50 & 69.89 & 70.14 & 4.80
& 27.54 & 38.89 & 31.78 & 34.88 & 32.20 & 0.00
& 35.54 & 74.05 & 63.16 & 66.16 & 64.32 & 5.76
& 33.33 & 71.31 & 59.69 & 63.37 & 50.00 & 5.88 \\

Gemini 3.1 Pro 
& 26.54 & 30.08 & 23.12 & 28.41 & 52.08 & 13.60
& 22.22 & 28.52 & 20.62 & 27.84 & 47.92 & 9.60
& 15.22 & 18.40 & 13.95 & 18.60 & 44.07 & 0.98
& 17.50 & 28.34 & 21.07 & 26.56 & 47.72 & 11.67
& 16.67 & 28.12 & 19.38 & 26.74 & 47.46 & 11.76 \\

\midrule

Gemini 3.1 Flash 
& 58.02 & 55.01 & 78.75 & 72.73 & 84.72 & 12.00
& 47.53 & 52.16 & 61.25 & 68.75 & 64.58 & 6.40
& 28.26 & 24.21 & 27.91 & 26.74 & 44.92 & 0.00
& 36.34 & 50.71 & 67.85 & 60.52 & 69.26 & 7.64
& 33.33 & 49.67 & 64.34 & 52.33 & 65.25 & 7.84 \\

DeepSeek-V4-Pro 
& 34.57 & 65.59 & 61.88 & 67.61 & 80.56 & 18.40
& 30.86 & 61.73 & 61.25 & 65.91 & 72.22 & 10.40
& 20.29 & 46.33 & 41.86 & 50.00 & 74.58 & 0.98
& 25.21 & 61.52 & 59.70 & 63.32 & 76.14 & 11.99
& 22.46 & 60.25 & 58.91 & 62.79 & 75.42 & 11.76 \\

\midrule

DeepSeek-V4-Flash 
& 31.48 & 53.08 & 71.88 & 65.91 & 82.64 & 11.20
& 28.40 & 50.78 & 68.75 & 65.34 & 75.00 & 6.40
& 22.46 & 36.51 & 43.41 & 41.86 & 68.64 & 0.00
& 26.81 & 50.48 & 69.54 & 62.59 & 76.49 & 7.12
& 25.36 & 49.95 & 68.99 & 61.05 & 72.88 & 5.88 \\

Qwen3.6-Max 
& 58.02 & 40.29 & 98.75 & 96.02 & 0.00 & 13.60
& 52.47 & 38.18 & 90.62 & 75.57 & 0.00 & 8.00
& 31.88 & 24.59 & 44.19 & 15.70 & 0.00 & 0.00
& 37.71 & 38.23 & 92.58 & 61.81 & 0.00 & 9.38
& 34.78 & 38.04 & 89.15 & 48.26 & 0.00 & 9.80 \\

Qwen3.6-Plus 
& 53.70 & 39.65 & 81.25 & 93.18 & 52.08 & 20.80
& 33.95 & 36.06 & 76.88 & 86.36 & 44.44 & 12.00
& 12.32 & 20.59 & 40.31 & 38.95 & 41.53 & 0.00
& 29.43 & 35.68 & 79.93 & 79.89 & 47.23 & 13.30
& 28.99 & 35.37 & 80.62 & 71.51 & 46.61 & 11.76 \\

Qwen3.6-27B 
& 0.00 & 1.75 & 15.62 & 19.89 & 0.00 & 0.00
& 0.00 & 1.75 & 13.75 & 18.75 & 0.00 & 0.00
& 0.00 & 1.33 & 6.98 & 9.88 & 0.00 & 0.00
& 0.00 & 1.75 & 14.08 & 16.96 & 0.00 & 0.00
& 0.00 & 1.72 & 13.95 & 15.12 & 0.00 & 0.00 \\

\midrule

Qwen3.6-35B-A3B 
& 46.30 & 34.87 & 28.12 & 44.89 & 35.42 & 13.60
& 38.27 & 31.00 & 22.50 & 43.75 & 29.17 & 4.80
& 18.12 & 15.63 & 9.30 & 15.70 & 29.66 & 0.00
& 28.12 & 30.06 & 21.58 & 36.05 & 31.96 & 5.53
& 26.09 & 28.98 & 19.38 & 27.91 & 30.51 & 4.90 \\

Gemma-4-31B 
& 56.17 & 39.56 & 83.12 & 66.48 & 77.78 & 12.80
& 42.59 & 37.17 & 66.25 & 61.36 & 61.81 & 8.80
& 25.36 & 16.30 & 25.58 & 25.58 & 64.41 & 0.00
& 34.86 & 35.49 & 67.16 & 56.64 & 69.07 & 9.60
& 33.33 & 34.99 & 63.57 & 52.91 & 66.10 & 7.84 \\

\midrule

Gemma-4-26B-A4B 
& 58.02 & 45.08 & 67.50 & 80.11 & 77.08 & 3.20
& 40.12 & 41.12 & 53.75 & 76.14 & 64.58 & 2.40
& 23.19 & 16.40 & 20.93 & 30.23 & 53.39 & 0.00
& 34.34 & 38.85 & 57.11 & 67.34 & 71.75 & 2.93
& 33.33 & 37.65 & 51.94 & 56.98 & 70.34 & 2.94 \\

Llama-4-Maverick 
& 46.91 & 33.95 & 22.50 & 21.02 & 4.17 & 21.60
& 37.04 & 29.25 & 17.50 & 18.75 & 3.47 & 10.40
& 21.74 & 11.92 & 3.88 & 8.14 & 4.24 & 0.00
& 31.32 & 25.58 & 19.14 & 15.22 & 4.24 & 12.03
& 28.99 & 23.45 & 19.38 & 13.37 & 4.24 & 10.78 \\

\midrule

Llama-4-Scout 
& 33.95 & 1.10 & 3.12 & 27.84 & 6.94 & 0.00
& 25.93 & 0.74 & 2.50 & 18.75 & 4.86 & 0.00
& 13.77 & 0.38 & 2.33 & 3.49 & 4.24 & 0.00
& 20.15 & 0.65 & 2.90 & 10.60 & 4.84 & 0.00
& 18.84 & 0.67 & 2.33 & 6.98 & 4.24 & 0.00 \\

Kimi K2.6 
& 6.17 & 4.42 & 1.88 & 3.98 & 0.69 & 4.00
& 4.94 & 3.96 & 1.88 & 3.41 & 0.69 & 0.80
& 3.62 & 3.43 & 2.33 & 2.91 & 0.85 & 0.00
& 5.09 & 3.95 & 2.33 & 3.43 & 0.85 & 0.98
& 5.07 & 3.91 & 2.33 & 3.49 & 0.85 & 0.98 \\

\midrule

Kimi K2 
& 58.02 & 41.67 & 50.00 & 7.39 & 31.25 & 22.40
& 45.06 & 39.83 & 44.38 & 7.39 & 25.69 & 16.00
& 27.54 & 24.21 & 23.26 & 4.65 & 18.64 & 0.98
& 34.98 & 38.39 & 42.26 & 7.25 & 24.67 & 18.47
& 32.61 & 37.75 & 41.09 & 6.98 & 22.88 & 16.67 \\

Doubao-Seed-2.0-Lite 
& 58.02 & 47.19 & 65.62 & 85.23 & 6.94 & 16.00
& 48.15 & 43.97 & 63.12 & 82.39 & 6.94 & 8.00
& 29.71 & 30.60 & 34.11 & 54.65 & 4.24 & 0.00
& 37.11 & 43.79 & 65.68 & 78.48 & 8.47 & 9.31
& 34.78 & 43.28 & 64.34 & 76.16 & 8.47 & 8.82 \\

Doubao-Seed-2.0-Mini 
& 7.41 & 0.83 & 0.00 & 0.00 & 0.00 & 11.20
& 7.41 & 0.74 & 0.00 & 0.00 & 0.00 & 7.20
& 5.80 & 0.38 & 0.00 & 0.00 & 0.00 & 1.96
& 6.73 & 0.75 & 0.00 & 0.00 & 0.00 & 8.53
& 6.52 & 0.76 & 0.00 & 0.00 & 0.00 & 8.82 \\

\bottomrule
\end{tabular}
}
\caption{Per-language evaluation results on PerfCodeBench. For each metric, results are reported separately for C, C++, Go, Java, Python, and CUDA. CRR denotes the correct-and-runnable rate; FBR denotes the faster-than-baseline rate; RBR denotes the reference-or-better rate; CGRE denotes correctness-gated relative efficiency; and CGRE$_{\ge 0.8}$ denotes the fraction of tasks closing at least 80\% of the baseline-to-reference performance gap.}
\label{tab:perfcodebench_results_by_language}
\end{table*}

